Langevin Monte-Carlo Provably Learns Depth Two Neural Nets at Any Size and Data

In this note we prove that the Langevin Monte Carlo (LMC) algorithm can minimize the population risk of appropriately regularized depth-2 nets with no restrictions on the size of the net and for any choice of training data --- and we give non-asymptotic convergence rates for it. We achieve this via showing that in q-Renyi divergence, the iterates of LMC converge to the Gibbs distribution of certain Frobenius norm regularized losses for these nets --- in both classification and regression settings. The key technicality of the work is two-fold (a) to keep the amount of regularization needed be independent of the size of the net and (b) to obtain convergence rates that scale with just the Poincare constant of the corresponding Gibbs measure. This work synthesizes several recent observations about isoperimetry conditions under which LMC converges and that two-layer neural loss functions can always be regularized by a constant amount such that they satisfy the Villani conditions, and thus their Gibbs measures satisfy a Poincare inequality.

==> Sections/Isoperimetry.tex <==
\section{Isoperimetric Inequalities}\label{app:sec:isoperimetry}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Images/Isoperimetry.png}
    \caption{A summary of the isoperimetric inequalities we discuss in this work.}
    \label{fig:isoperimetry}
\end{figure}

% \note{Put a diagram showing PI, LOI and LSI.}

\subsection{Log-Sobolev implies \Poincare inequality}\label{appendix:LSI-PI}

% \note{Refer to Bakry et. al. --- this is a standard result known in ??, which we are reproducing for readers convenience.}

For completeness we reproduce the standard result that distributions with satisfy the Log-Sobolev inequality also satisfy the Poincare inequality \cite{handel2016probability}. 
%for completeness.
\newline
\newline
The LSI, for a test function $f \geq 0$ can be written as,
\begin{align}\label{eq:lsipi}
    \Ent_\pi [f] \leq 2 C_{LSI} \E_\pi[\langle \grad \sqrt{f}, \grad \sqrt{f} \rangle]
\end{align}
where $\Ent_\pi[f] \coloneqq \E_\pi[f \log f] - \E_\pi[f] \log \E_\pi[f]$.The RHS of the above inequality can be simplified in the following manner,
\begin{align*}
    &2 C_{LSI} \E_\pi[\langle \grad \sqrt{f}, \grad \sqrt{f} \rangle] = 2 C_{LSI} \E_\pi\left[\left\langle \frac{\grad f}{2\sqrt{f}}, \frac{\grad f}{2\sqrt{f}} \right\rangle\right] \\
    = &\frac{C_{LSI}}{2} \E_\pi\left[\left\langle \frac{\grad f}{f}, \grad f \right\rangle\right] = \frac{C_{LSI}}{2} \E_\pi\left[\left\langle \grad \log f, \grad f \right\rangle\right]
\end{align*}
Without loss of generality we can replace $f$ by $e^{\lambda f}$ for some $\lambda \geq 0$ to get,

% \note{refer to equation \ref{eq:lsipi} and give the full definition of Ent here before substituting }

\begin{align}
    \E_\pi[\lambda f e^{\lambda f}] - \E_\pi[e^{\lambda f}] &\log \E_\pi[e^{\lambda f}] \label{app:mlsi_pi:eq1} \\
    &\nonumber\leq \frac{C_{LSI}}{2} \E_\pi[\langle \grad \lambda f, \grad e^{\lambda f} \rangle]
\end{align}

As $\E_\pi[\langle \grad f,\grad 1 \rangle] = 0$, we can say from Taylor expanding $e^{\lambda f}$
\begin{align*}
    \E_\pi[\langle \grad \lambda f, \grad e^{\lambda f}\rangle] = \lambda^2 \E_\pi[\langle \grad f, \grad f\rangle] + \gO(\lambda^3)
\end{align*}
For the terms in the LHS of the inequality in equation \ref{app:mlsi_pi:eq1} we have,
\begin{align*}
    \E_\pi[\lambda f e^{\lambda f}] = \lambda \E_\pi[f] + \lambda^2 \E_\pi[f^2] + \gO(\lambda^3)
\end{align*}
% \note{isn't the error term $o(\lambda^3)$?}
and
\begin{align*}
    &\E_\pi[e^{\lambda f}] \log \E_\pi[e^{\lambda f}]\\
    &= \left(1 + \lambda \E_\pi[f]\right) \left(\log (1 + \lambda\E_\pi[f] + \frac{\lambda^2}{2}\E_\pi[f^2]) \right) + \gO(\lambda^3)\\
    &= \left(1 + \lambda \E_\pi[f]\right) \left(\lambda \E_\pi[f] + \frac{\lambda^2}{2} \E_\pi[f^2] - \frac{\lambda^2}{2} (\E_\pi[f])^2 \right) + \gO(\lambda^3)\\
    % &\text{\color{red} what is the expansion of log used above?}\\
    &= \lambda\E_\pi[f] + \lambda^2\{ \E_\pi[f^2] + \E_\pi[f]^2 \}/2 + \gO(\lambda^3)
\end{align*}
% \note{this is not clear as to what happened above!}
Replacing the above three perturbative expansions into equation \ref{app:mlsi_pi:eq1} we get,
\begin{align*}
    \frac{\lambda^2(\E_\pi[f^2] - \E_\pi[f]^2)}{2} + \gO(\lambda^3) \leq \frac{C_{LSI}}{2} \lambda^2\E_\pi[\langle \grad f, \grad f \rangle] + \gO(\lambda^3)
\end{align*}
Dividing both sides by $\lambda^2$ and letting $\lambda \to 0$ we get,
\begin{align*}
    \Var[f] \leq C_{LSI} \E_\pi[\langle \grad f, \grad f \rangle]
\end{align*}
%\note{this is not an argument! in the $\lambda \rightarrow 0$ limit all terms disappear as given here - i think one needs to do a better counting of the lambda terms and substitute all expansions back into equation \ref{app:mlsi_pi:eq1} and compare the two sides of the equation}
which is the \Poincare inequality w.r.t the arbitrary test function chosen at the beginning.
